Identifying Cause-and-Effect Relationships of Manufacturing Errors using Sequence-to-Sequence Learning

In car-body production the pre-formed sheet metal parts of the body are assembled on fully-automated production lines. The body passes through multiple stations in succession, and is processed according to the order requirements. The timely completion of orders depends on the individual station-based operations concluding within their scheduled cycle times. If an error occurs in one station, it can have a knock-on effect, resulting in delays on the downstream stations. To the best of our knowledge, there exist no methods for automatically distinguishing between source and knock-on errors in this setting, as well as establishing a causal relation between them. Utilizing real-time information about conditions collected by a production data acquisition system, we propose a novel vehicle manufacturing analysis system, which uses deep learning to establish a link between source and knock-on errors. We benchmark three sequence-to-sequence models, and introduce a novel composite time-weighted action metric for evaluating models in this context. We evaluate our framework on a real-world car production dataset recorded by Volkswagen Commercial Vehicles. Surprisingly we find that 71.68% of sequences contain either a source or knock-on error. With respect to seq2seq model training, we find that the Transformer demonstrates a better performance compared to LSTM and GRU in this domain, in particular when the prediction range with respect to the durations of future actions is increased.

==> sections/abbreviations.tex <==
\thispagestyle{plain}
\addsec{List of Abbreviations}
\label{sec:listOfAbbreviations}
\begin{acronym}[Identifying cause-and-effect relationships of manufacturing errors using attention based neural networks]
  \acro{AI}{Artificial Intelligence}
  \acro{CSV}{comma-separated values}
  \acro{HDF5}{Hierarchical Data Format} %version5
  \acro{MSE}{Mean Squared Error}
  \acro{PSNR}{Peak Signal-to-Noise Ratio}
\end{acronym}


==> sections/background.tex <==
\section*{Background}

\comJR{overview subsection to be written last in this section.}
% In this section, the important concepts in this paper are presented. The anomalies of chained manufacturing systems and the effects are explained so that the importance of predicting anomalies can be explained. For this purpose, existing approaches to LSTM are presented and compared. In the next section, the functionality and structure of the LSTM technique are described, and the applicability and advantages of LSTM are explained. Finally, a look at basic methodological concepts for the application of machine learning methods is provided.

\subsection*{Interlinked manufacturing system} \label{sec:interlinked_manufactring system}
\comJR{sounds generic, is it still good for talking about car body assembly?}

In 1994, U. Klages described a form of interlinked manufacturing system.
In interlinked manufacturing systems, especially transfer lines for large-scale production of, for example, automotive parts, the individual machining units are often connected via a rigid transport system.
The transfer lines are generally used to manufacture exactly one workpiece in large quantities.
The transport system ensures the simultaneous transport of the workpieces from machining unit to machining unit of the transfer line.
However, it also couples the processing units in such a way that all processing units must function together in order to ensure the function of the overall transfer line system. \cite{KLAG94}
Nowadays, there are already more flexible manufacturing systems.
In [GRUN04] a definition of a flexible manufacturing system (FMS) is presented: "A flexibly interlinked multi-machine system in which several complementary or substituting CNC machines, usually machining centres, measuring machines and others, are linked via a computer-aided workpiece transport system.
\comJR{reference [GRUN04] is missing!}
The automatically operated workpiece storage systems for raw and finished parts are also partly linked to the transport system".
This description is suitable for interlinked manufacturing systems in this work.

%\subsection{Time Series Data} \label{sec:time_series_data}



% A definition of time series is provided by Keogh Eamonn in 2007: 
% Time-series: "A time series T = t1.... tm is an ordered set of m real-valued variables". Time series data are formed according to the order of the points in time at which they are created \cite{KEOG06}.  
% Therefore, time series data should be understood as data corresponding to a fixed sequence of time numbers within a certain time interval (2 years, 6 months, etc.). 

%  J. Frausto et al. built a prediction model of oil production time series data and explained that if the sequence of observations from a time series is expressed by x(T) (T = t1, t2, ...), then the expression x(T+h) denotes the prediction horizon for period h at time T, where h = 1 means one step ahead and h > 1 means a prediction several steps ahead \cite{FRAU15}.




% \subsection{Basic methodological concepts for the application of machine learning methods}
\comJR{data scientists would know about "Basic methodological concepts for the application of machine learning methods", or?}
% For some time now, the disruptive effects of digitalisation on the future viability of existing business models, but also on changes in entire industrial sectors and the economy as a whole, have been discussed.
% It is already evident today that value chains are breaking up and being reconfigured.
% Digital platforms enable new business concepts, companies increasingly operate simultaneously in several networks.
% Digitalisation is not only changing the industrial landscape, but also labour markets, urban infrastructure, mobility, housing and our social life.
% Ultimately, all these changes would not be possible without new technologies that allow an accelerating growing volume of data to be recorded, evaluated and used in various ways \cite{BRÜH19}.
% An overview of the connections between Big Data, data mining (DM), machine learning (ML) and predictive analytics is given in Figure 2 .3. 

% Efforts in the industrial domain mainly concern the definition of processes / methods that can guide the implementation of DM applications. The most popular models are KDD (Knowledge Discovering in Database), SEMMA (Sample, Explore, Modify, Model, Assess) and CRISP-DM (Cross-Industry Standard Process for Data Mining) because they are presented in many publications and really used in practice~\cite{AZEV08}.

% All ML methods require a large data set and depend on the quality of the features. In addition, different types of data (such as time series data) will greatly influence the methods used. In this paper, CRISP-DM is chosen as the guidance method because CRISP-DM (see in Figure 2 .4) is more complete than SEMMA and easy to understand \cite{AZEV08}. Before applying the ML method for data analysis and so on, the following requirements should be met: 

% \begin{enumerate}
% \item Business understanding - This first phase focuses on understanding the project goals and requirements from the business perspective, and then transforming this knowledge into a data mining problem definition and a preliminary plan to achieve the goals.
% \item Data understanding - The data understanding phase begins with initial data collection and continues with activities to become familiar with the data, identify data quality issues, gain initial insights into the data or identify interesting subsets to form hypotheses for hidden information. 
% \item Data preparation - The data preparation phase includes all activities to create the final data set from the initial raw data. 
% \item Modelling - In this phase, different modelling techniques are selected and applied and their parameters are calibrated to optimal values.
% \item Evaluation - In this phase, the model (or models) obtained are evaluated more thoroughly and the steps performed to create the model are reviewed to ensure that the business objectives are properly achieved. 
% \item Deployment - The creation of the model is generally not the end of the project. Even if the purpose of the model is to improve knowledge about the data, the knowledge gained needs to be organised and presented in a way that the client can use.  
% \end{enumerate}


==> sections/data.tex <==
\section*{Data preparation}
\comJR{statistische Signifikanz von Musterfehler erst im Kapitel data.tex erwähnen}
\comJR{erwähnen in data.tex über ob Störungsmeldungen vorliegne und wieviele}

\subsection{}


\subsection{Error labelling}

First, a file of "Time\_difference" of an action (e.g. R04 process) is imported.
There are only two columns, "Sequence" and "Time\_difference" (see Figure 4 .10).
"Sequence" stands for the series of this event in the associated action database and "Time\_difference" of course stands for the duration of the action.
There is a value of Time\_difference at every second row, because each action consists of a start event and an end event.
At the end event, the value of Time\_difference (as well as the duration of the action) is documented.

To simplify counting, all duration values are converted to integers.
By counting the number of occurrences of different durations, the duration with the most occurrences is obtained, i.e. the main peak or mode (see Figure 4 .11).
According to the sequence numbers, all data points from main peaks are found in the corresponding action database and marked as normal data. If only one duration is found, all data from that action will be considered normal. 

The next step is to find the correct second peak.
To do this, a theoretical normal distribution (Gaussian distribution) is sought that fits the existing data distribution.
To fit a distribution curve, the maximum likelihood estimation (MLE) method is required.
The density function of the normal distribution contains two important parameters: expected value  $\mu$  and standard deviation $\sigma$(.
These two parameters determine the shape of the density function and the probability corresponding to a point in the distribution. 

\comGP{Insert eq 4.10}
\begin{equation} \label{eq:4.1_from_original}
f(x \mid \mu, \sigma^2) = \frac{1}{\sqrt{2\pi\sigma^2}} \exp\left(-\frac{(x-\mu)^2}{2\sigma^2}\right)    
\end{equation}

The method of MLE is a parametric estimation procedure that can estimate two parameters of density function that the determined distribution seems most plausible according to its distribution of the observed data.
\comGP{Variables need to be inserted}
MLE assumes an observed variable whose density function depends on two unknown parameters $\mu$ and $\sigma$(together as below).
The density function describes the magnitude of the probability of coming from a distribution with.
The joint density function can be factorised as follows: 

\comGP{eq 4.2}
\begin{equation} \label{eq:4.2_from_original}
f(x_1, x_2, ..., x_n \mid \vartheta) = \Pi^n_{i=1}f(x_i \mid \vartheta)
\end{equation}

For a fixed observed variable, the joint density function of can be interpreted.
This leads to likelihood function: 

\begin{equation} \label{eq:4.3_from_original}
L(\vartheta) = \Pi^n_{i=1}f_\vartheta(x_i)
\end{equation}

The value of $\vartheta$ is sought for which the sample values $x_1, x_2, ..., x_n$ have the largest density function.
This is obvious, the higher the likelihood, the more plausible a parameter value $\vartheta$ is.
As long as the likelihood function is differentiable, the maximum of the function can be determined.
Thus, the parameters $\mu$ and $\sigma^2$ obtains.

In this work, all data of duration of an action are to be understood as the variables $X$.
Moreover, the mode, i.e. the duration with the most occurrences, is defined as the expected value $\mu$.
This leaves only one unknown parameter, the standard deviation $\sigma$.
The implementation of the determination of $\sigma$ in Python is shown as in the appendix (see Figure 8 .35).

After this, the parameters as well as the normal distribution for the corresponding data and the total probability density function are determined.
If the proportion of the number of occurrences of a duration to the total data exceeds the value of the corresponding probability density function, the data with this duration are selected as data from second peak (as well as third peak, etc.) or as potential original errors. 

Next, the selected data is compared with the data in the error message database, e.g. whether the start and end time of the error is within the period of the action and whether the information of the error such as Area and Station matches the information of the action. All corresponding data are marked as original errors and the rest are marked as drag errors. In addition, the number of the error is also documented. (see the two rightmost columns in Figure 4 .12)

In the context of this work, we only focus on the actions in station 7240 with vehicle number 0021. Finally, all action data are marked as normal, original error, dragging error and undefined according to the above steps. In addition, each action forms a new file with label. 

\textbf{Integrate Training Data}

After error labelling, all files with label are integrated so that we can get a new raw production database with label. Thus, a training database is generated with action number, error type label and number of error (Figure 4 .13).

\subsection{Modelling}

\textbf{Pre-processing of the training data}

Initially, only all rows with AC number in the training database are selected. Such rows contain the timestamp and duration of the associated action, which defines a time period of the action. Therefore, the rows with event number are no longer required. Then the columns like Station and Car Code are deleted. In this work, only the data from station 7240 with Car Code 0021 is considered. In the future, data from other station with different car type will be added. In addition, the lines with AC 000, 006 and 013 are excluded. These actions stand for "Takt", "Rob 05 Prozess" and "Rob 04 Prozess" respectively (see Figure 4 .8). 

The action Takt describes a complete action sequence of a vehicle in station 7240. The action Rob 05 Prozess and Rob 04 Prozess describe all production actions of Robot 05 and Robot 04 respectively. It leads to overlapping information and negative impact on the training of the model because the training database contains every action information. But AC 000 (clock) will remain temporary and still play a role in the next steps. 

Next, all data is left integer or unchanged as needed and finally normalised. The timestamp is processed as the number of seconds that have passed since 01.01.2020. The Event is converted as an integer from 0 to the number of actions. For error type, normal, original error, drag error and undefined are each to be understood as an integer from 1 to 4. The data of Time\_diff(s) and Error Count remain unchanged. The processed database is shown as in Figure 4 .14. 

\comGP{4.14}

At the same time, the number of data with different error types in training data is better represented (see Figure 4.15).

\comGP{4.15}

After pre-processing the database, a total of 162,339 rows of data are obtained, including 89,465 normal actions, 20,817 drag errors, 664 original errors and 51,393 undefined data. 

\textbf{Filtering outliers or outlier sequence}

In practice, there are outliers of duration that are oversized. Such data can have a negative impact on the training of the model, although it seems rare. The probable causes may be downtime during holidays or random failure. To minimise this impact, all data defined as outliers are excluded. There is no basic maximum duration (Max. Duration) of the action yet. Therefore, different Max. Duration (e.g. 600, 400, 200 seconds) are set. This is disadvantageous to delete each of these dates because the original sequence of actions is changed. 

An alternative is to exclude all production sequences that contain the outlier. The action clock i.e. AC 000 is to be understood as the beginning of a production sequence. Therefore, a production sequence is defined by two continuous AC 000. There is an example of a production sequence with an outlier (see Figure 4 .16). 

\comGP{4.16}

After eliminating the outlier (AA), numerous rows of data are deleted. With a maximum duration of 600 seconds, 1,167 rows of data are filtered. After eliminating the production sequences with outliers (APS), a total of 14,835 rows of data are filtered. This is acceptable because of the huge amount of data (162,339 rows in total). Chapter 5 compares the performance of the models under AA and models under APS. In addition, the effect of different maximum allowed durations is discussed. The overview of the filtered data under different maximum durations is presented in Table 4.1.

\comGP{Table 4.1}

\begin{table}[]
\large%

\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|}

\hline
\textbf{Editing} & \textbf{Number of filtered data} & \textbf{Proportion of filtered data (total 162,339)} & \textbf{Max. Duration (seconds)} \\
\hline
\hline
AA & 1.167 & 0,72\% & 600 \\
\hline
APS & 14.835 & 9,14\% & 600 \\
\hline
AA & 1.688 & 1,04\% & 400 \\
\hline
APS & 21.529 & 13,26\% & 400 \\
\hline
AA & 3.745 & 2,31\% & 200 \\
\hline
APS & 49.035 & 30,21\% & 200 \\
\hline
\end{tabular}}
\caption{The number of filtered data under different durations}
\label{tab:The_number_of_filtered_data_under_different_durations}
\end{table}



\textbf{Normalisation and listing according to the number of look-back steps}
In the next step, all data are normalised from -1 to 1 to allow calculation in LSTM unit. Then a pattern for the prediction of the LSTM model is designed. It is desired that the model looks 3 ,5 or more steps in the past and then predicts the next two actions and their duration. Therefore, a listing of the processed database must be performed to achieve a desired shape (e.g. 3 look-back steps and 2 steps in the future):

\comGP{insert plot}

The number here only represents the order of the action, instead of the actual action number. Each Act\_x here is to be understood as a row of the processed training database.
This is implemented in Python (see Figure 8 .36) and the result is shown below (Figure 4 .17).

\comGP{Figure 4.17}

The data in Figure 4 .17 is not yet normalised for better understanding. The variables 1 to 5 are respectively timestamp, action number, duration, error type and error count. Only the next 2 action numbers and associated durations are predicted (var2 and var3). This is the final processed data. 

The first 3 steps or 15 rows of data (from t-3 to t-1) will be understood as the input to LSTM model and the last 2 steps or 4 rows (from t to t+1) of data will be understood as the correct solution of prediction. In case of discrepancies between the output of the LSTM model and the correct solution, the LSTM tries to adjust the neural weights to obtain a higher accuracy.
Finally, the data is divided into training and testing data. In this paper, the first 80\% data is considered as the training data and the last 20\% data is considered as the test data.

The amount of data in the training data and test data varies depending on the previous processing method (e.g. AA or APS, number of look-back steps). For example, the data is processed with APS. After listing, there are 110,085 rows of training data and 27,520 rows of test data. (see Table 4 .2)

\comGP{Table 4.2}

\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Processing} &
\textbf{Review steps} &
\textbf{Training data} &
\textbf{Test data}  \\
\hline
\hline
AA & 3 & 121.351 & 30.336 \\
\hline
APS & 3 & 110.087 & 27.520 \\
\hline
AA & 5 & 121.349 & 30.336 \\
\hline
APS & 5 & 110.085 & 27.520 \\
\hline
AA & 7 & 121.348 & 30.335 \\
\hline
APS & 7 & 110.084 & 27.519 \\
\hline
\end{tabular}}
\caption{Amount of training data and test data}
\label{tab:Amount_of_training_data_and_test_data}
\end{table}

\textbf{Separation of the new vehicle}
As told in section 4.1, the vehicles to be produced always enter the station one after the other until they are produced. It is possible to perform a separation between different vehicles. If there are different types of vehicles in the future database, it will be necessary to make separation between vehicles. The implementation is described below. 
Assume that a production sequence contains from Act\_1 to Act\_9. When Act\_1 is displayed, it means that a new vehicle comes to the station for production and the previous vehicle has finished production. The separation is done like this: 

\comGP{figure}

\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l||l|l|}
\hline
Act\_5 & Act\_6 & Act\_7 & Act\_8 & Act\_9 \\
\hline
Act\_6 & Act\_7 & Act\_8 & Act\_9 & empty \\
\hline
Act\_7 & Act\_8 & Act\_9 & empty & empty \\
\hline
Act\_1 & Act\_2 & Act\_3 & Act\_4 & Act\_5 \\
\hline
… & … & … & … & … \\
\hline
\end{tabular}}
\caption{Example of the separation.}
\label{tab:Amount_of_training_data_and_test_data}
\end{table}

In section 4.3.1 it is mentioned that AC 000 should remain short. AC 000 is to be understood here as the first action as well as Act\_1. This makes the lines with AC 000 the breakpoint lines. After the separation, the lines with AC 000 are also excluded.

It will be proved in the following work that such separation has a positive effect on the quality of the prediction. Therefore, the model without separation and the model with separation will be compared in the next chapter.

The set-up is shown below. (see figure 4 .18)

\comGP{Figure 4.18}

The amount of training data and test data is changed after separation. The change can be observed in Table 4.3. 

\comGP{table 4.3}

\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l||l|l|}
\hline
Processing & Separation & Retrospective steps & Training Data & Test Data\\
\hline
AA & Yes & 3 & 106.177 & 26.543 \\
\hline
APS & Yes & 3 & 95.747 & 23.935 \\
\hline
AA & Yes & 5 & 91.007 & 22.750 \\
\hline
APS & Yes & 5 & 81.410 & 20.351 \\
\hline
AA & Yes & 7 & 75.843 & 18.959 \\
\hline
APS & Yes & 7 & 67.080 & 16.768 \\
\hline
\end{tabular}}
\caption{Amount of training data and test data after separation .}
\label{tab:Amount_of_training_data_and_test_data_after_separation}
\end{table}

\subsection{Creating the LSTM model}
\comJR{irrelevant section (?)}

Keras is an open-source deep learning library with intuitive code and clear feedback written in Python. Keras library makes it quick and easy to create an LSTM model.

It is important to set appropriate hyperparameters of the model, for example, the number of layers (hidden layers), nodes (nodes), etc. Suitable parameters play a positive role in various tasks. At the same time, the choice of parameters is also a difficult problem in building machine learning models. Currently, it is not easy to determine the appropriate optimal parameters based on existing tasks. Therefore, a preliminary experiment is conducted in this paper to determine the initial parameters. Next, these parameters are adjusted in the experiment.

In other literature, a model with 2 LSTM layers and 80 nodes is built to detect the anomaly of a robotic system \cite{DING20}. In the preliminary experiment of this work, it is tried to build models with 2 to 4 LSTM layers and 50 to 100 nodes. After referring to similar work and preliminary experiments, the parameters of 4 LSTM layer and 50 nodes are selected. 

The activation function for output layer is tanh (see Figure 4.19). This function has an amplitude from -1 to 1. It is explained why all data are normalised from -1 to 1 earlier. 

For the loss function, "MAE" (mean absolute error) is selected and the optimiser is "Adam" (adaptive moment estimation). The closer the predicted result is to the actual value, the better the predictive ability of the model. Under MAE Loss function, the absolute deviation between predicted and actual value is calculated. Adam is a commonly used deep learning optimisation algorithm, which is used here for training to minimise MAE.

To control the training time of the model within an acceptable range, the model is trained with 50 epochs and 128 batch-size. The batch-size is the number of samples of training data in each iteration. The number of iterations is the total number of training data divided by the batch-size. 1 epoch means that all iterations are completed. Theoretically, there is an optimal batch-size under a fixed number of epochs. If the batch-size is too small, it is possible that the loss function will no longer converge. On the contrary, if batch-size is too large, more epochs will be needed. This will lead to an increase in time.

After preliminary tests, 128 batch-size is found to be a relatively good parameter among 50 epochs. The training time is 5 to 6 minutes. 
The visualisation of the model, the result of the training and the code in Python are shown below. (Figure 4 .20, Figure 4 .21 and Figure 8 .37)

\comGP{Figure 4.20 (move to supplementary material.}

\comGP{Figure 4.21}

When training the model, it turns out that increasing the number of nodes in the model has a positive effect on the results. Therefore, an experiment was set up and the models were grouped according to the factors mentioned in the previous section (such as Steps, Separation, Max. Duration, AA and APS) and their performances were compared. (see Table 4 .4)

\comGP{Table 4.4}
\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
No.  & Name & Separation & Review steps (Steps) & Node & AA & APS & Max. Duration \\
\hline
1  &
OT\_Model\_1 &
Nein &
3 &
50 &
Nein &
Nein & \\
\hline
2 &
OT\_Model\_2 &
Nein &
3 &
50 &
Ja &
Nein &
600 \\
\hline
3 &
OT\_Model\_3 &
Nein &
3 &
50 &
Nein &
Ja &
600 \\
\hline
4 &
T\_Model\_1 &
Ja &
3 &
50 &
Nein &
Nein & \\
\hline
5 &
T\_Model\_2 &
Ja &
3 &
50 &
Ja &
Nein &
600 \\
\hline
6 &
T\_Model\_3 &
Ja &
3 &
50 &
Nein &
Ja &
600 \\
\hline
7 &
T\_Model\_1\_5s &
Ja &
5 &
75 &
Nein &
Nein & \\
\hline
8 &
T\_Model\_2\_5s &
Ja &
5 &
75 &
Ja &
Nein &
600 \\
\hline
9 &
T\_Model\_3\_5s &
Ja &
5 &
75 &
Nein &
Ja &
600 \\
\hline
10 &
T\_Model\_3\_5s\_1 &
Ja &
5 &
100 &
Nein &
Ja &
600 \\
\hline
11 &
T\_Model\_3\_5s\_2 &
Ja &
5 &
150 &
Nein &
Ja &
600 \\
\hline
12 &
T\_Model\_3\_5s\_3 &
Ja &
5 &
200 &
Nein &
Ja &
600 \\
\hline
13 &
T\_Model\_3\_5s\_4 &
Ja &
5 &
100 &
Nein &
Ja &
400 \\
\hline
14 &
T\_Model\_3\_5s\_5 &
Ja &
5 &
100 &
Nein &
Ja &
200 \\
\hline
15 &
T\_Model\_1\_7s &
Ja &
7 &
100 &
Nein &
Nein & \\
\hline
16 &
T\_Model\_2\_7s &
Ja &
7 &
100 &
Ja &
Nein &
600 \\
\hline
17 &
T\_Model\_3\_7s &
Ja &
7 &
100 &
Nein &
Ja &
600 \\
\hline
\end{tabular}}
\caption{Numbers and names of the models for experiment.}
\label{tab:numbers_and_names_of_the_models_for_experiment}
\end{table}


==> sections/empirical_evaluation_comment.tex <==
% \section*{Empirical Evaluation} \label{sec:empirical_eval}


% \subsection*{Experiment design}

% As mentioned in chapter 4, an experiment is conducted to find factors of optimal influence and associated model. All the differences of the models are found in Table 4 .4.

% At the beginning, the models without separation are compared with models after separation. At the same time, the difference of the models after AA or APS is considered. They are trained all the time under the same parameters and looking back 3 steps, so that it can be proved whether model without separation is better or model after separation is better. (see Table 4.4, Models 1-6).

% After that, it is determined for further experiments whether the model is trained with or without separation. 

% Next, the models with lookback of 5 steps and models with lookback of 7 steps are compared (see Table 4 .4, Models 7-9 and 15-17). If there are different lookback steps, the nodes will also be different. If there are more lookback steps, the nodes of each LSTM layer also become more, e.g. if there are 5 lookback steps, 75 nodes are needed. 
% After comparing all the models, the model with best fit is selected. It is also determined whether the model is trained after separation, AA or APS. Finally, it is checked how the model behaves with different nodes and maximum durations (see table 4 .4, models 10-14)



% \subsection*{Experimental results}
% \comGP{Move "(in our case it is 60s)" down to section 7.}.

% \textbf{General suitability of different models}
% After training the model with the training data, the model must be verified with the test data. Test data is data that never appears during the training process of the model. Therefore, the reliability and robustness of the model are checked. 
% Here, model no. 10 (T\_Model\_3\_5s\_1) is taken as an example. Partial prediction is shown in Figure 5 .22. 

% From the figure 5 .22 it can be seen that most of the action numbers are predicted correctly. Furthermore, the predicted duration is also close to the actual value as long as the action number is predicted correctly. It is worth noting that the model does not predict the position of separation well. Moreover, the prediction for t has better quality than the prediction for t+1.

% To evaluate the quality of the prediction, the accuracy and Root Mean Square Error (RMSE) are used as criteria. Accuracy explains how many percentages of actions are correctly predicted. The RMSE is a measure to assess the prediction quality of the duration. The higher the accuracy, the better and the lower the RMSE, the better. 

% In this comparison, models 10 to 14 are excluded first, as they are all based on the changes of model 9. Later they are compared with model 9. The accuracies and RMSEs of the different models are shown below (see Figure 5 .23 and Figure 5 .24). 

% The observations lead to the following conclusion: 

% \begin{enumerate}
% \item First, it becomes obvious that models after separation have better accuracy and lower RMSE than models without separation (model 1-3 compared to model 4-6). This verifies that separation has a positive effect on the fit of the model.

% \item Secondly, the RMSE of the model after AA or APS is much lower than RMSE of the model without AA or APS (model 1 vs. model 2-3). The associated accuracy also becomes a little better or the same. This makes it clear that AA or APS can improve the quality of the prediction.

% \item Subsequently, it can be seen that the models according to APS are slightly better than the models according to AA. With AA, the data on maximum duration is filtered directly. The original action series is destroyed. This leads to poorer accuracy and RMSE.

% \item Finally, it is observed that the models (models 7-9) with look-back steps of 5 have the best accuracy on average. At the same time, these models (models 8-9) have similarly good RMSE according to AA or APS compared to the models with look-back steps of 3 and 7 (models 5-6 and models 16-17). 
% \end{enumerate}


% With 7 look-back steps, the length of the training data is shortened too much (see Table 4 .3). This affects the fit of the trained model. Therefore, look-back steps of 5 is selected as the best. 
% This leads to the conclusion that the model 9 is the best performing of these models. The model is trained after separation and APS with maximum duration of 600. The look back step is 5 and the node is 75. 
% There is an opportunity to improve the fitness of the 9th model. In the following, it is tried to train new models with different nodes and different maximum durations based on model 9 with the other parameters unchanged (models 10-14). They are then compared with each other. 
% Here new evaluation criteria are added, RMSE for duration below 60 seconds (see Figure 5 .27). In raw database there are 145,646 rows of data with duration less than 60 seconds. The proportion of these data is 89.72\%. Therefore, it is a significantly important assessment whether the model has lower RMSE for data with durations below 60 seconds. Furthermore, when comparing models with similar fit, it is more difficult to distinguish between high and low according to the RMSE of the entire data. The results of models 10-14 compared to model 9 are shown below (see Figure 5 .25, Figure 5 .26 and Figure 5 .27).

% Figure 5.25 shows that models 10-12 have better accuracies than the other models. Model 12 has the best accuracy. On the contrary, models 13 and 14 have relatively worse accuracies. The reason is that too much data is filtered at maximum duration of 400 or 200 (see Table 4 .1). If the training data set is shortened too much, the goodness of the model's prediction is also weakened. 

% The RMSEs of models 9-13 are fairly close. For models 13-14, the RMSEs naturally become lower because the associated maximum duration is smaller. When evaluating RMSEs for durations below 60s, Model 10 takes first place.

% It is difficult to say which model has a better fit because the values of accuracy and RMSE of the models can be very close. There is no possibility to work with established evaluation criteria (e.g. Precision and Recall) yet. Therefore, a special evaluation method will be developed, which will be understood here as a score of the model. The formula for the score is as follows:
% \par
% \comYD{Note = 0.6 $\times (0.7 F1score_t + 0.3 F1score_{t+1}) \times 100 + 0.4 \times F(n,k) (n=2, k=15, a_n=[0.7,0.3])$}
% \par
% \comYD{Replace G1 for actions with the F1 score of predictions.}

% \begin{equation} \label{eq:5.1_from_dissertation}
% Note = 0.6 \times (0.7 G_t + 0.3 \times G_{t+1}) \times 100 + \par  0.4 \times \frac{1}{15} \times \{0.7 \times (15 - R_t) + 0.3 \times (15 - R_{t+1})\} \times 100 
% \end{equation}

% \hspace*{\fill} \\


% The and stand for precision of t and t+1. The and mean the RMSE for duration under 60s of t and t+1. In addition, precision has a weight of 0.6 and RMSE (under 60s) has a weight of 0.4. All predictions for t have a weight of 0.7 and predictions for t+1 has a weight of 0.3. 15 is a reference value of RMSE (under 60s). The total score is 100. Compared to RMSE, accuracy is considered a more important evaluation criterion. The prediction of t becomes more important than the prediction of t+1.

% As can be seen from Figure 5 .28 above, Model 10 has the highest score. Model 10 is considered the best model.

% The result of the No.10 model is shown in Table 5 .5. 

% \comGP{Table 5.5}


% \begin{table}[]
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% Model no. & Accuracy (t) & RMSE (t) Under 60s  & Accuracy (t+1) & RMSE (t+1) Under 60s   & Note \\
% \hline
% 10 & 86,60\% & 6,805 & 77,50\% & 7,164 & 71,89 \\
% \hline
% \end{tabular}}
% \caption{Model 10 result.}
% \label{tab:Model_10_result}
% \end{table}

% \textbf{Statistical validation of the best model results}

% In order to validate the stability of the model training process, it is necessary to perform multiple repeated training so that the variations in the model prediction results can be observed.

% In this paper, model number 10 is repeatedly trained 10 times under the same parameters. The change in accuracy and RMSE is documented and shown in Figure 5 .29 and Figure 5 .30. 

% In addition, the fluctuation of the grade is also recorded (see figure 5 .31).

% The mean values of the results are presented in Table 5 .6.

% \comGP{Table 5.6}

% \begin{table}[]
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% Model Nr. &
% Accuracy (t) &
% RMSE (t) Under 60s &
% Accuracy (t+1) &
% RMSE (t+1) Under 60s  &
% Note \\
% \hline
% 10 &
% 86,52\% &
% 7,353 &
% 76,78\% &
% 7,373 &
% 70,53 \\
% \hline
% \end{tabular}}
% \caption{Mean values of the results of model 10.}
% \label{tab:Model_10_result}
% \end{table}

% For repetitive training, the maximum change in accuracy is 3.06\% and the maximum change in RMSE is 3.669. The variation in accuracy is minor. At RMSE (below 60s) and grade, there are two worst models, the 4th and 9th models. 

% The result of each training is basically stable. But there is a possibility that the trained model has relatively worse RMSE (below 60s). 

% \textbf{Analysis of the fit of model 10}

% Model-10's fit of predicting action is relatively stable. However, there is relatively violent fluctuation in the prediction of duration. It is reflected in the RMSE (below 60s). This leads to the question why there is such fluctuation in prediction of duration.

% There are two ways to find the answer. 
% The calculation under LSTM model is responsible for this. 
% There are combinations of data in the test data that the model has never seen during training.

% In this paper, the second possibility is checked. The following Figure 5 .32 and Figure 5 .33 show the change in RMSE (under 60s) after each additional 500 lines of predicted data for each model. The models are referred to as models W1 to W10. 

% It is obvious that RMSE (below 60s) often has a violent jump after 2500 lines. After that, RMSE (below 60s) is reduced again and stable to a certain extent. In contrast to RMSE for t, RMSE for t+1 is always relatively balanced. 

% The observations lead to the following conclusion that there are combinations of data in the test data between 2500 and 3000 rows that the model did not encounter before during training. 

% One particular combination is found (see Figure 5 .34). It is verified in Python that this combination never appears in training data. 

% This combination (after AC 012 comes AC 015) is not in the processed training data. At the same time, the associated durations are also abnormal.  The duration for AC 012 is usually less than 1 second and action 015 also rarely occurs in the test data. The model predicted incorrectly for AC 015 and over-predicted both durations. Similar situations were observed in the predictions of other models. But in model W2 and W3, there are only minor jumps.

% This leads to the conclusion that this combination is most likely the cause of the jump. 


==> sections/motivation.tex <==
% \section{Motivation}

% Nowadays, AI has brought new opportunities in various industries. In traditional industries such as engineering, a huge amount of production data has been accumulated. With the help of machine learning model (like LSTM), this production data is analysed to optimise the production process. This can maximise the value of the data. 
% Also, by predicting anomalies in production, the time to check stations can be reduced, improving production efficiency.


==> sections/problem_def_comments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% https://arxiv.org/pdf/1702.03037.pdf

% https://www.ncbi.nlm.nih.gov/pmc/articles/PMC4033239/#:~:text=4.2.-,Semi\%2Dmarkov\%20decision\%20process,occur\%20at\%20discrete\%20time\%20steps.&text=This\%20process\%20is\%20called\%20semi,the\%20action\%20has\%20been\%20taken.

% See section 4.2 for definition of semi-MDP, which operates on continuous time. 

% Production time series data and explained that if the sequence of observations from a time series is expressed by $x(T) (T = t_1, t_2, ...)$, then the expression $x(T+h)$ denotes the prediction horizon for period $h$ at time $T$, where $h = 1$ means one step ahead and $h > 1$ means a prediction several steps ahead \cite{FRAU15}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Objective Function}\label{objective_function}

% The \acl{MSE} is a measure to indicate how good a predicton of an action is and is compared always to the ground truth.
% \[MSE = \frac{1}{n}\sum_{i=1}^{n}(\widehat{Y_{i}}-Y_{i})^{2}\]
% Similar to lossy image compression the \ac{MSE} itself is not capable to describe the severity of the error without knowing the upper limit of possible value.
% By taking the peak value into account, the \acl{PSNR} does not have this problem and it is defined as followed:
% \[PSNR = 10 \log_{10}(\frac{MAX_{i}^{2}}{MSE})\]
% while \(MAX_{i}\) equals 600, since 600s is the upper limit of possible predictions of time in our work.
% \comJR{ToDo: citation needed!}



% Sowohl die Ausgabe bzw. Vorgabe einer Zielzeit sowie die Einhaltung dieser Zeit sind zwei wesentliche \acl{KPI} in der Produktion.
% Für unseren Use-case ist es daher vom wesentlichen Interesse, dass ein Modell zur Prädiktion der Zeiten nicht nur global, d.h. prädizierten Zeiten aller Aktionen einschließlich die über der max Toleranz Zeit sind, ein Minimum erreicht wird.
% Viel eher ist die Prädiktion der Zeiten von Sequenzen innerhalb der max Toleranz Zeit vom wesentlichen Interesse, weil üblicherweise viele Musterfehler Zeiten nicht weit entfernt von der Zielzeit sind.
% Daher wird hier die eine neue Metrik eingeführt, die besonders berücksichtigen wie die Güte der Prädiktion innerhalb der max Toleranz Zeit ist.
% Die Anzahl an Prädiktionen in die Zukunft ist variable, daher verwenden wir einen Faktor $\alpha_{i} = e^{-i}$ bei der die Güte der unmittelbaren Prädiktion mehr Gewicht trägt als Nachkommende.
% Die Skalierungswert $k$ orientiert sich dabei an einen zu erwartenden Zeit.
% Diese Zeit wird durch die gegenwärtige Prädiktion $R_{t_i}$ subtrahiert.
% Resultierend ergibt sich dabei folgende Funktion:






% \subsection{Error propagation}
% \comJR{need to explain cause-and-effect relationships of manufacturing errors and them going over various stations?}

%%%%%%%%%%%% old here %%%%%%%%%%

% \subsection{Anomalies in Time Series Data of Interlinked Manufacturing Systems}

% Anomaly is a term with many different contents. It is easy to confuse the definitions of anomaly, fault and error. Therefore, it becomes necessary to clearly explain the definition of anomaly in computer science, statistics or time series data and distinguish it from the definition of fault in manufacturing or quality management. 
% One definition is provided by Xu. Anomaly detection in time series data is the identification of data points that do not match expected patterns in a data set. Such as, intrusions detection in cybersecurity, fraud attempts detection in financial transactions and diseases diagnosis in public health \cite{XU18}. Similarly, N. Davis also defined the anomalies in time series data that the time series data with anomalies have the pattern that does not correspond to a certain expected behaviour. In Transportation Networks, there are some cases where anomalous patterns and behaviour occur. For example, sudden spikes in taxi demand could indicate the end of a concert, a drop in traffic speed could be the result of an unprecedented event such as a traffic accident, and so on \cite{DAVI19}. 

% An anomaly is thus understood as an unexpected event or sudden change in the state of a system of observation that leads to normally negative effects on the system of observation. 

% Furthermore, anomalies in time series data are described by other English literature: "Anomalies unexpected in time series data can be the results of amplitude change or shape change" [ZHOU21]. In other words, an anomaly in time series data can be understood as a large change in the shape or amplitude of some time series data compared to most other data. 

% In 2009, J. Schumacher presented the disturbances and disturbance management in production. A disruption only occurs when a process deviates from its planned course. Examples of such disruptions are missed deadlines, machine downtimes, tool breakage, missing material, employees falling ill or sudden quality defects \cite{SCHU09}. These examples have summarised the cause and effect of disruptions. In addition, terms for malfunction are described in other literature: "In production engineering, a malfunction is therefore understood to be a temporary unintentional suspension or an unacceptable reduction in the qualitative and/or quantitative performance of a production facility. Malfunctions are subdivided according to their causes ... and reduce the availability of the system" \cite{GRIE81}.

% In the context of this work, a malfunction is to be understood as an interruption of the functionality or avoidance of the availability of the manufacturing system due to technical or organisational causes. In contrast to the definition of anomaly, the definition of disruption is a more precise case of anomaly. For example, an anomaly can be caused by the slowing down of a process, which leads to the slowing down of the whole system. In this case, it is not recognised as a disorder. 
% Next, it is important to understand what anomalies are likely to occur in time series data of chained manufacturing systems and how they affect the system.

% \comJR{info: Adjacent work from students is in progress here: 1)Categorization of Anomalies in Industrial Production, 2) List and Compare ML Detection Methods in Industrial Production;
% Something useful to take away from it or need to adjust direction of students?
%]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]]ubsection{Impact of anomalies}

% In the English literature, there is a potential impact of anomalies in 
% linked manufacturing systems called "sequence scrambling". M. Lehmann has illustrated the whole automotive manufacturing system and the phenomenon of "sequence scrambling". It is not possible to effectively apply the car sequencing rules directly at the beginning of the production process, i.e. in the body shop where the orders are released into the system, because the sequence is generally mixed during the manufacturing process.  Highly customised cars, prototypes, quality samples, rework, downtime and non-synchronised production steps lead to deterministic and stochastic lead time extensions during the manufacturing process. Therefore, several cars fall behind while others overtake, which changes the initial sequence during the production process.  This phenomenon is called sequence scrambling \cite{LEHM20}. In the context of this work, sequence scrambling plays only a small role, because the main anomalies occur after the sequence is set. In addition, sequence scrambling is caused by external factors such as missing parts. They hinder the proper assembly of the vehicle in such a way that the vehicle either cannot be built at all or the missing parts have to be retroactively installed in the rework area \cite{LEHM20}. This rework is likely to cause a significantly higher effort and thus higher costs, as the parts are not installed during their specified production step. It is also considered that sequence scrambling is a cause of the anomaly of following production. 

% The theory of the butterfly effect is well known. Here it refers to the effect that in some systems small causes can have large, mostly unpredictable effects \cite{SCHU09}. Schumacher also provides an example: "For example, a small metal chip in the oil can cause the oil pump to fail. The result is an overheated machine bearing, which eventually leads to a machine malfunction. As a result, deadlines are missed, which in turn leads to a penalty and a poor supplier rating" [SCHU09/206]. 

% Accordingly, when anomalies occur, the effects are usually referred to as delaying a consideration system, decreasing productivity and increasing production costs. In the context of this work, such delays will occur at independent workstations of the interlinked manufacturing systems. These delays not only have an original effect on the station itself, but also have a detrimental effect on the downstream stations. To prevent and reduce these negative effects, it becomes necessary to detect and predict relevant anomalies. 

% \subsection{Prediction of anomalies}

% Machine learning (ML) is a subfield of artificial intelligence (AI). The term AI describes machines that behave as if they had some kind of human intelligence. The complex algorithms of ML were not established until the 1990s. With the popularisation of Big Data in various industries, the ML model has a lot of training data. When AlphaGo, a computer programme developed by Google, defeated a professional Go player for the first time in 2016, one of the key successes of ML was achieved. This has also brought Deep-Learning to people's attention and inspired more and more researchers. Deep-learning is one of the algorithms of ML that mimics the multi-layer neural unit network of humans so that the machine can assess the problem with thinking similar to humans. \cite{WELS18} 

% The significant progress that deep learning methods have made in recent years on various ML problems has encouraged researchers to explore them for anomaly detection as well. Thanks to the vast amounts of data being discovered and used, deep-learning algorithms can make connections between different data and outcomes to make predictions that are more accurate than humans. The suitability of deep learning models for anomaly detection and prediction is due to their unsupervised learning nature and ability to learn highly complex nonlinear sequences. \cite{DAVI19}
% In [MALH15], two methods, LSTM and Recurrent Neuron Network (RNN), are used to detect and predict anomalies in four real-world data types.  In the paper, it is shown that LSTM and RNN methods are equally good for the data sets without long-term temporal dependency (such as "Electrocardiograms, Multi-sensor engine data"). On the other hand, LSTM shows significant improvement over RNN for datasets with long-term time dependence as well as short-term dependence (e.g. "Space-Shuttle Valve time series, Power demand dataset"). On average, LSTM models have better Precision, Recall, and Scorce than RNN models. The formulas for Precision, Recall, and -Scorce are presented as (2.1), (2.2) and (2.3). [MALH15/94] 

% \comGP{Perhaps too much info for a journal, even for the appendix}
% \comJR{requires a check on target venue papers how far they go in detail about anomalies, if at all? If none existant, we need it}

% % \begin{equation} \label{eq:precision}
% % Precision = \frac{TP}{TP+FP}    
% % \end{equation}


% % \begin{equation} \label{eq:precision}
% % Recall = \frac{TP}{TP+FN}    
% % \end{equation}

% % \begin{equation} \label{eq:precision}
% % F1 = \left(\frac{1/Precision+1/Recall}{2}\right)^{-1}    
% % \end{equation}

% In computer science, the prediction of anomalies in time series data for application metrics is studied with the aim of performing anomaly detection and system resource management \cite{JERO18}.  To this end, Jerome et al. implemented a collection of models, including an LSTM model, ETS (Exponential Smoothing) and ARIMA (Autoregressive Integrated Moving Average), and compared their performance. The prediction bounds for the LSTM model's anomaly identification predictions are established. For various evaluation criterion, the prediction of LSTM model performed well \cite{JERO18}. 

% Anomaly detection is used for industrial automation system. Lindemann and his colleagues have applied the LSTM autoencoder to detect anomalies in large amount of machine and process data. They have also compared it with the k-means clustering method and found that the LSTM autoencoder tracks more accurately for anomalies \cite{LIND19} .  It is worth noting that Ding provides a statement that the quality of the dataset used for LSTM model training is very important. Poor quality training datasets lead to a decrease in the prediction accuracy of the LSTM model and even incorrect predictions or detections \cite{DING20}.

% On the other hand, anomalies in interlinked manufacturing system often do not occur independently but influence each other. The previous anomaly may be the cause of the next anomaly \cite{LEHM20}. Up to now, there are no methods to classify anomalies into original and subsequent defects and to establish a link between them and to evaluate the significance of an original defect. Furthermore, it is expected that this procedure will be used to predict the occurrence of the next anomalies or next production state. The complexity of this task also poses challenges for machine learning modelling (such as LSTM).
% In summary, LSTM performs better than other methods in detecting and predicting time series data anomalies. However, at the same time, a higher quality data set is required to train the model. Therefore, the necessary adjustments to the LSTM model must be made based on the existing dataset. The following part describes the functionality and structure of LSTM in detail.

% \subsection{LSTM}
% \comJR{if also including TadGAN as an approach here, we need a section to discuss why we choose only two out of how many approaches?\\
% maybe further in conclusion reference to Transformers as a possible next step to iterate on LSTM?}

% \comGP{No need to re-introduce LSTMs in detail. At the most include in supplementary material, but not really necessary.}
% \comGP{Some variables did not transfer from the text while copying and pasting.}

% When training the RNN, the vanishing gradient problem occurs but lacks effective solution \cite{SOUT13}. The LSTM network is a special type of RNN proposed by Hochreiter et al. to overcome the vanishing gradient problem \cite{JERO18}.
% All recurrent neural networks take the form of a chain of repeating neural network modules. In standard RNNs (see in Figure 2 .1), this repeating module has a very simple structure, such as a single tanh layer \cite{OLAH15}.


% LSTMs also have this chain-like structure, but the repeating module has a different structure. Instead of having just one neural network layer, there are four that interact in a very particular way. In Figure 2 .2, , and denote the input, the hidden state and the cell state at time . In this figure, represents the forget/remember gate output, which controls how much of the previous cell state is transmitted. In the current time step, we calculate a candidate cell state . The input gate controls how much of this candidate cell state is combined with to produce. The output gate and the current cell state determine the value of the hidden state \cite{JERO18}.

% For the LSTM cell, the use of peephole connections is investigated and better performance is found. As shown in equation (2.4), (2.5), (2.8), peephole connections allow the LSTM unit to look into the cell state while calculating the output of the forgetting gate, input gate and output gate \cite{JERO18}.
% In [DING20/218-220], a whole normal dataset and dataset with manual input errors are used. The dataset used in this paper has the characteristics of large size, real collection and many undetected anomalies. Therefore, necessary adjustments are required.
% Before training an LSTM model, it is necessary to set appropriate values for various hyperparameters. These parameters define the higher-level features of the model, such as its complexity or its learning ability. In an LSTM model, the important hyperparameters are, for example, the number of hidden recurrent layers, the dropout values, the learning rate and the number of units in each layer. \cite{DAVI19} 

% \subsection{Understanding data}

% Body construction means the precise assembly of several hundred individual parts made of steel and aluminium of different sizes and thicknesses to form a precision body. Depending on the vehicle requirements, carbon and fibre composites are also used in addition to steel and aluminium. In production, the car body passes through many stations one after the other. At each station, many robots will process them according to the order requirements, and when processing is complete, they will be passed on to the next station. The shop floor data collection system (PDA system) collects and documents all real-time information. From this data, an online Gantt chart can be generated to visually show the time spent in each production step (see figure 4 .7). 

% In the production database (see Figure 3.5), columns such as Area, Section, Station, Timestamp, Event, Time\_Difference and more information can be found. The information such as Timestamp and Event are constantly updated after information such as Area and Station in the online mode on Gantt Chart. Each data line describes the current production event at the corresponding time. Each action results from two events, a start event and an end event. The crucial definitions are shown in Figure 4.8.

% The information from Area, Section, Station describes the location of the production event. Time\_Difference only occurs at the end of the action, which indicates the duration of the action. The timestamp of End-Event and the duration of the action define the period of an action. The code can be used to generate a separate data file for each action. In this way, each action can be analysed separately. 

% The duration (Time\_Difference) of each action is counted and ordered. A histogram based on number of durations is shown to observe the number of occurrences of different durations and their distribution. (see figure 4 .9)

% Theoretically, a normal distribution is expected. If there is only one main peak in the histogram, all data points of this main peak are to be understood as normal data. Otherwise, unwanted further peaks appear in the histogram. These represent significant accumulations of errors. The underlying cause-effect relationships must therefore at least be learned by the LSTM.
% In the context of this work, different errors are to be understood as anomalies. All raw production and error message data of the car body production come from a large German car manufacturer. To achieve a better understanding, the following definitions of different defect types are given.

% \textbf{Pattern defects: }

% When these defects occur with statistical significance, i.e. the defects are not random, these defects are understood as pattern defects. The unwanted peaks or peaks in the histogram are assumed to be such errors because they do not conform to the normal distribution around a stationary desired time. The peaks are assumed to contain original and drag errors.

% \textbf{Original errors (origin errors):}

% All data points of a peak are checked to see if there are corresponding entries in the error message database. For each data point, the corresponding search period in an error message database should be set to identify if, how many and which errors are found. If one or more errors are found, then the data point is classified as an original error. 

% \textbf{Tracking error (following error):}

% If no error is found when matching a data point from a peak with the error message database, then this is classified as a tracking error. It is then assumed that a preceding original error is responsible for the tracking error.

% Before LSTM can learn these relationships, all data would have to be labelled accordingly. The data is divided into normal data, original errors and tracking errors. For example, in Figure 4.3 there is a very obvious main peak with more than 1750 data points with a duration of 30 seconds. The data points of the main peak are all marked as normal. In addition, there is a notable second peak with 1218 data points with a duration of 36 seconds. All data points of this peak must be checked to see if there are corresponding entries in the error message database. If one or more errors are found, then the data point is classified as an original error. Other data points of this peak are then defined as drag errors. The rest are marked as undefined data. Finally, all marked data from different actions are sorted into time series and used as training and test data for training the LSTM model.

% In the next step, the implementation is presented.

==> sections/table_original.tex <==
\begin{center}[]
\begin{table*}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{14}{|c|}{Setup 5-2} \\
% \hline
\hline
\textbf{Model} &
$\mathbf{RMSE_1}$ &
$\mathbf{RMSE_2}$ &
$\mathbf{F1_1}$ &
$\mathbf{F1_2}$ &
$\mathbf{TARMSE}$ &
$\mathbf{F1}$ &
$\mathbf{CTA}$  \textbf{(\%)}\\
\hline
\textbf{GRU 5-2} &
$4.14 \pm 0.24$ &
$4.12 \pm 0.63$ &
$0.94 \pm 0.02$ &
$0.95 \pm 0.01$ &
$0.20 \pm 0.05$ &
$0.94 \pm 0.01$ &
$59.89 \pm 3.02$ \\
\hline
\textbf{LSTM 5-2} &
$4.01 \pm 0.39$ &
$4.06 \pm 0.49$ &
$0.95 \pm 0.01$ &
$0.95 \pm 0.01$ &
$0.22 \pm 0.08$ &
$0.95 \pm 0.01$ &
$58.49 \pm 4.08$ \\
\hline
\textbf{Transformer 5-2} &
$2.95 \pm 0.02$ &
$3.29 \pm 0.05$ &
$0.80 \pm 0.02$ &
$0.82 \pm 0.03$ &
$0.41 \pm 0.01$ &
$0.80 \pm 0.01$ &
$60.55 \pm 0.76$ \\
\hline
\end{tabular}}
\caption{Setup 5-2}
\label{tab:Model_5-2_result}
\end{table*}
\end{center}

\begin{table*}[]
%\resizebox{\columnwidth}{!}{
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
Model &
$RMSE_1$ &
$\mathbf{RMSE_2}$ &
$\mathbf{RMSE_3}$ &
$\mathbf{RMSE_4}$ &
$\mathbf{RMSE_5}$ &
$\mathbf{F1_1}$ &
$\mathbf{F1_2}$ &
$\mathbf{F1_3}$ &
$\mathbf{F1_4}$ &
$\mathbf{F1_5}$ &
$\mathbf{TARMSE}$ &
$\mathbf{F1}$ &
$\mathbf{CTA}$ \textbf{(\%)} \\
\hline
\multicolumn{14}{|c|}{Setup 5-5} \\
\hline
\textbf{GRU 5-5} &
$4.07 \pm 0.18$ &
$3.72 \pm 0.29$ &
$3.50 \pm 0.18$ &
$3.51 \pm 0.23$ &
$4.29 \pm 0.41$ &
$0.94 \pm 0.02$ &
$0.95 \pm 0.02$ &
$0.89 \pm 0.03$ &
$0.89 \pm 0.01$ &
$0.92 \pm 0.01$ &
$0.24 \pm 0.02$ &
$0.94 \pm 0.02$ &
$58.67 \pm 1.33$ \\
\hline
\textbf{LSTM 5-5 }&
$4.03 \pm 0.21$ &
$3.88 \pm 0.21$ &
$3.84 \pm 0.30$ &
$3.68 \pm 0.34$ &
$4.09 \pm 0.53$ &
$0.94 \pm 0.02$ &
$0.94 \pm 0.01$ &
$0.89 \pm 0.02$ &
$0.90 \pm 0.01$ &
$0.93 \pm 0.01$ &
$0.23 \pm 0.03$ &
$0.93 \pm 0.01$ &
$58.11 \pm 1.53$ \\
\hline
\textbf{Transformer 5-5 }&
$3.04 \pm 0.02$ &
$2.70 \pm 0.02$ &
$2.43 \pm 0.02$ &
$2.35 \pm 0.02$ &
$2.77 \pm 0.06$ &
$0.79 \pm 0.03$ &
$0.81 \pm 0.02$ &
$0.79 \pm 0.03$ &
$0.80 \pm 0.01$ &
$0.78 \pm 0.02$ &
$0.44 \pm 0.00$ &
$0.80 \pm 0.02$ &
$61.69 \pm 0.85$ \\
\hline
% \end{tabular}}
% \caption{Setup 5-5}
% \label{tab:Model_5-5_result}
% \end{table}

% \begin{table}[]
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{14}{|c|}{Setup 7-5} \\
\hline
% \hline
% Model &
% $RMSE_1$ &
% $\mathbf{RMSE_2}$ &
% $\mathbf{RMSE_3}$ &
% $\mathbf{RMSE_4}$ &
% $\mathbf{RMSE_5}$ &
% $\mathbf{F1_1}$ &
% $\mathbf{F1_2}$ &
% $\mathbf{F1_3}$ &
% $\mathbf{F1_4}$ &
% $\mathbf{F1_5}$ &
% $TARMSE$ &
% $F1$ &
% $CTA$  (\%) \\
\hline
\textbf{GRU 7-5} &
$3.99 \pm 0.22$ &
$3.97 \pm 0.19$ &
$4.09 \pm 0.41$ &
$3.77 \pm 0.35$ &
$4.23 \pm 0.52$ &
$0.89 \pm 0.03$ &
$0.89 \pm 0.02$ &
$0.94 \pm 0.01$ &
$0.94 \pm 0.01$ &
$0.92 \pm 0.01$ &
$0.22 \pm 0.03$ &
$0.89 \pm 0.02$ &
$55.83 \pm 2.12$ \\
\hline
\textbf{LSTM 7-5} &
$4.08 \pm 0.32$ &
$4.15 \pm 0.35$ &
$4.21 \pm 0.24$ &
$3.92 \pm 0.34$ &
$4.29 \pm 0.84$ &
$0.91 \pm 0.04$ &
$0.90 \pm 0.02$ &
$0.94 \pm 0.01$ &
$0.94 \pm 0.01$ &
$0.92 \pm 0.03$ &
$0.20 \pm 0.04$ &
$0.91 \pm 0.03$ &
$55.80 \pm 2.19$ \\
\hline
\textbf{Transformer 7-5} &
$2.68 \pm 0.04$ &
$2.55 \pm 0.02$ &
$2.59 \pm 0.02$ &
$2.57 \pm 0.04$ &
$2.78 \pm 0.10$ &
$0.81 \pm 0.01$ &
$0.81 \pm 0.02$ &
$0.81 \pm 0.01$ &
$0.81 \pm 0.01$ &
$0.75 \pm 0.02$ &
$0.49 \pm 0.01$ &
$0.81 \pm 0.01$ &
$64.75 \pm 0.59$ \\
\hline
\end{tabular}}
\caption{Setup 7-5}
\label{tab:Model_7-5_result}
\end{table*}

\begin{table*}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}

\hline
\multicolumn{18}{|c|}{Setup 7-7} \\
\hline
\hline
\textbf{Model} &
$\mathbf{RMSE_1}$ &
$\mathbf{RMSE_2}$ &
$\mathbf{RMSE_3}$ &
$\mathbf{RMSE_4}$ &
$\mathbf{RMSE_5}$ &
$\mathbf{RMSE_6}$ &
$\mathbf{RMSE_7}$ &
$\mathbf{F1_1}$ &
$\mathbf{F1_2}$ &
$\mathbf{F1_3}$ &
$\mathbf{F1_4}$ &
$\mathbf{F1_5}$ &
$\mathbf{F1_6}$ &
$\mathbf{F1_7}$ &
$\mathbf{TARMSE}$ &
$\mathbf{F1}$ &
$\mathbf{CTA}$ \textbf{(\%)} \\
\hline
\textbf{GRU 7-7} &
$4.10 \pm 0.32$ &
$4.00 \pm 0.29$ &
$4.24 \pm 0.41$ &
$4.06 \pm 0.28$ &
$4.15 \pm 0.27$ &
$3.49 \pm 0.31$ &
$3.28 \pm 0.24$ &
$0.87 \pm 0.04$ &
$0.89 \pm 0.03$ &
$0.91 \pm 0.02$ &
$0.93 \pm 0.02$ &
$0.85 \pm 0.04$ &
$0.85 \pm 0.03$ &
$0.85 \pm 0.04$ &
$0.21 \pm 0.05$ &
$0.88 \pm 0.02$ &
$54.24 \pm 3.58$ \\
\hline
\textbf{LSTM 7-7} &
$4.05 \pm 0.40$ &
$4.07 \pm 0.26$ &
$4.30 \pm 0.16$ &
$3.82 \pm 0.32$ &
$4.15 \pm 0.29$ &
$3.51 \pm 0.98$ &
$3.68 \pm 0.56$ &
$0.92 \pm 0.02$ &
$0.90 \pm 0.01$ &
$0.93 \pm 0.01$ &
$0.94 \pm 0.01$ &
$0.89 \pm 0.02$ &
$0.88 \pm 0.04$ &
$0.88 \pm 0.03$ &
$0.21 \pm 0.05$ &
$0.92 \pm 0.01$ &
$56.22 \pm 2.55$ \\
\hline
\textbf{Transformer 7-7} &
$2.72 \pm 0.03$ &
$2.56 \pm 0.02$ &
$2.57 \pm 0.03$ &
$2.57 \pm 0.02$ &
$2.66 \pm 0.05$ &
$2.86 \pm 0.06$ &
$2.70 \pm 0.07$ &
$0.80 \pm 0.01$ &
$0.80 \pm 0.02$ &
$0.79 \pm 0.01$ &
$0.79 \pm 0.01$ &
$0.75 \pm 0.02$ &
$0.72 \pm 0.02$ &
$0.76 \pm 0.03$ &
$0.48 \pm 0.00$ &
$0.80 \pm 0.01$ &
$63.88 \pm 0.70$ \\
\hline
\end{tabular}}
\caption{Setup 7-7}
\label{tab:Model_7-7_result}
\end{table*}
